RealityEffects: Augmenting 3D Volumetric Videos with Object-Centric Annotation and Dynamic Visual Effects

This paper introduces RealityEffects, a desktop authoring interface designed for editing and augmenting 3D volumetric videos with object-centric annotations and visual effects. RealityEffects enhances volumetric capture by introducing a novel method for augmenting captured physical motion with embedded, responsive visual effects, referred to as object-centric augmentation. In RealityEffects, users can interactively attach various visual effects to physical objects within the captured 3D scene, enabling these effects to dynamically move and animate in sync with the corresponding physical motion and body movements. The primary contribution of this paper is the development of a taxonomy for such object-centric augmentations, which includes annotated labels, highlighted objects, ghost effects, and trajectory visualization. This taxonomy is informed by an analysis of 120 edited videos featuring object-centric visual effects. The findings from our user study confirm that our direct manipulation techniques lower the barriers to editing and annotating volumetric captures, thereby enhancing interactive and engaging viewing experiences of 3D volumetric videos.

==> trash.tex <==
% Adding Object-Centric Annotation and Visual Effects to 3D Volumetric Videos
% Editing 3D Volumetric Videos with Dynamic Visual Effects and Annotations


INTRODUCTION

% Our study suggests that the edited volumetric video increase the engagement and memorability of such a video in education, training, and tutorial scenarios.

% by conducting a conditional experiment with Unity, so that we can compare how our system provides a better support for video editing and capturing.

% reduces the time to create a simple video editing, but also increases the expressiveness of the volumetric videos. 
% We have also conducted the evaluation for audience point of view, where we measure how such an annotated volumetric video increases the audience engagement. 



% , which allows the authoring the dynamic effects without programming.


% \item Two user studies that measures the effectiveness of Recorded Reality from editors' and audience perspective.
% \item Demonstration of application scenarios, such as sport training, physics education, classroom tutorials, and xxx. 
% that can reduce the time and efforts for video editing and annotation, enabled by the new object tracking techniques that combines computer vision and 3D volumetric video. 
% that can seamlessly blend the dynamic visual effects with the captured physical environment.

% We believe more simple and intuitive authoring technique that allows the easy creation of augmented volumetric videos can open up the untapped potential of the immersive viewing experiences that leverage free-viewpoint movement, that is not possible in augmented 2D videos. 



% When adding the visual of annotation effects to volumetric videos require more demanding tasks, especially for novice users because the user needs to manipulate both time and spatial 3D scene, so that additional dimension may require the change of view, etc. 
% In the current practice, we learned that expert users often need to use 3D game engine like Unity or Blender to add these effects, but from the formative interview, these tools do not provide an easy-to-use and accessible ways to edit volumetric videos. 

% First, the system allows the user to add 1-1) object, 1-2) text, 1-3) line/geometry. 
% Second, the system allows the user to modify these elements for 2-1) translate, 2-2) transformation, and 2-3) visual parameter (opacity, color, speed).
% Third, these elements can be bound to 3-1) static, 3-2) object, 3-3) body.
% Based on these features, 

% 360-degree video, as known as surround video\cite{nielsen2005surround}, immersive video or spherical video, which is a genre of video content that leverages an omnidirectional camera or a collection of cameras to capture the scenes in every direction simultaneously---enabling the audience to view in any point of view within immersive environment during the playback. 


% With the rise of 360-degree video content, the demand for 6-DOF \emph{volumetric capture} is rising. 
% Volumetric videos are considered the next stage of the video content [cite]. Unlike the traditional "flat" 2D or 360-degree videos, volumetric videos offer the depth information provided with volume, allowing the end-user to view directly in mixed reality and explore the 3D scenes instead of viewing the video from a single, constant depth.
% Nowadays, AR and VR in particular drives the applications for volumetric capture, highlighting the potential for volumetric video across multiple industries, from music to VFX, to e-commerce and beyond.

% Volumetric capture involves using multiple depth cameras to film a subject, creating a full volume recording of the subject, rather than a flat image. Through post production, this captured volume data becomes a volumetric video, which is then viewable from any angle, with realistic depth, color and lighting, on any compatible platform, including mobile devices.

% Popular online video platforms such as YouTube firstly supported 360-degree videos back in 2015. And during that time, with the wide spread of Google Cardboard, which is a low-fi and do-it-yourself VR headset, 360-degree videos had been quickly adopted by the general public, especially the publishers, such as mainstream journalists and media brands.
% For example, the film---Vice News's Millions March NYC [cite] was the first-ever news story broadcast that engages the audience in the march through the smart phone and VR headset with the use of 360-degree video in early 2015.
% Nowadays, fully immersive, 360-degree video has become a hot commodity while the 360-degree video cameras (also known as spherical or omnidirectional camera) are more powerful and accessible than ever, and the viewing options are plentiful, from social media platforms to VR headsets. Such 360-degree immersive contents are widely adapted in a wide range of online videos, such as space exploration by NASA [cite], animal documentary by National Geographic [cite], a guided city tour in Rome [cite], and beyond.

% The big BUT is where a problem is introduced. Or, similarly, a problem can be framed as an opportunity. Whether you are solving a problem or seizing an opportunity, motivate your work by connecting it to things that matter to people.

% While some video platforms have developed compatibility features for further immersion, such 360-degree videos are still merely created for the immersive viewing experiences, which allow the HMD audience to view the video in both horizontal and vertical axis. 

% The use of the term "virtual reality" to describe 360-degree video has been disputed, as VR typically refers to interactive experiences wherein the viewer's motions can be tracked to allow real-time interactions within a virtual environment, with orientation and position tracking. In 360-degree video, the locations of viewers are fixed, viewers are limited to the angles captured by the cameras, and cannot interact with the environment. The non-dynamic nature of video also means that rendering techniques cannot be used to reduce the risk of motion sickness.

% Given these applications, we are now aware of the extent of these video tools and their limitations.


% During this century, we have seen the rise of mass media consumption. And with it, the development of many tools that aid in processing or creating them. Indisputably the most mainstream medium for these medias is in the form of a video. 


% With the development of specialized cameras and widespread of MR devices, commercial uses have been popularized. Looking at 360$^{\circ}$ videos or 3DOF videos. They provide immersion by allowing the ability to look around but lack any form of interactivity with the environment. While there has been exploration in more immersive forms of 360$^{\circ}$ spatial videos such as 6DOF videos using Canon EOS VR or Remixed Reality. But there still exists limited interactions with these videos. Mainly restricted to temporal or object interactions such as rewinding or object selection and manipulation.

% Further interactions such as annotation, sketching or editing could greatly benefit the experience handling 360$^{\circ}$ Spatial Videos. Much like post processing tools much like Insta360 Studio, After Effects or Premiere that support 360$^{\circ}$ Spatial Videos.

% And with that, we present Recorded Reality. A 360$^{\circ}$ Spatial Video editing tool capable of embedding annotations, sketching responsive visualizations and forms of video processing/filtering.

%After the big BUT, you will describe what you did, now in a bit more detail than in the Abstract. Devoting a paragraph to what you did is reasonable in the Introduction.

%Kevin - I'm not too sure what our workflow would look because I'm unsure about the implementation. Just some quick stuff I thought what the POC would look like.

% \begin{comment}
% Our approach incorporates the following workflow to implement our system. 1)Record(Record the spatial video using depth cameras) 
% 2)Selection + Tracking(User selection either of or from the environment and track either movement or colour)
% 3)Annotation(Embed text to selected aspects) + Sketching (Responsive visualizations with real world values)
% 4)Playback + viewing (Timeline maneuverability and POV change)
% 5)Data representation?(Extension of sketching by incorporating graphs? Like movement heatmaps or data extracted from sketches?)

% Some questions:
% What device/platform will our system be on?


% \end{comment}

%After saying what you did, you should offer the key results of what you did. What were the major findings? Whereas the Abstract might have devoted a sentence or two to key results, now you can devote a whole paragraph.

% \begin{comment}
% The applications:
% 1)Improve mainstream media consumption by increasing accessibility to immersive video viewing experiences(Might be contribution?)
% 2)Augmented physics experiments(Educational tool)
% 3)Expressive/creative video outlet(Cinematography?)
% \end{comment}

%Finally, a good way to end your Introduction is by framing the contributions that your work makes. (See “Seven Research Contributions in HCI” [12] for examples of different research contributions.) I often structure my contributions as a numbered list within a paragraph. “The main contributions of this work are: (1) ...; (2) ...; (3) ...”
% To summarize, our paper makes the following contributions:
% \begin{enumerate}
%   \item Recorded Reality, a video editing tool for authoring annotations, spatio-temporal responsive visualizations and video processing/filtering for 360$^{\circ}$ Spatial Videos. %Artifact contribution
%   \item A design space of the applications of our system revolving around practical uses such as education.(Expand once we decide on applications)
%   \item 
%  \end{enumerate}


% The Introduction delivers the motivation for your paper. It explains why you did the work you did. This is the primary function of the Introduction.

% • State of the world...
% • The big BUT...
% • Therefore, we did...
% • The key findings are...
% • The contributions of this work are...

% The state of the world is a description of issues in whatever “world” is relevant to your topic. Drawing on popular press can be effective here if recent news items or data from articles support your cause.

% Volumetric videos are considered the next stage of the video content, as a variation to the current hot commodity in media consumption---

% Volumetric video has many potentials and it has mant inte application areas, entertain , sport , tutorial and beyond. given that vol could be the next video platform



% Volumetric videos---a genre of video content that leverages an omnidirectional camera or a collection of cameras to capture the scenes in every direction simultaneously---enabling the audience to view in any point of view within immersive environment during the playback. 


% However, there are not so many tool for editing the vol video, unlike 2D video editing tool (AE..), editing  of volumetric video introduces lots of challenge, 
% for example the user has to interact in the 3d scene, requires a lot of 
% in a commercial product, there are some tools that are limited in terms of timeline manipulation, and if the user want to add visual of annotation effects, the user needs to use blender, etc... 
% current tool for vol editing such as ... only allows the user to navigate of modify ... but adding visual effects is still not well supported.
% The curent challenge is that the user has to navigate in space and time in 3d space, require additional dimension, requirs skills and time. And in this paper, address the paper by object-bound approach, to add effects and editing vol video by leveraging object-bound editing 



% 1st paragraph


% Today, we are living in an era of shifting from 2D to 3D worlds.
% For example, digital contents on screens are now becoming 3D with AR/VR glasses and interactions are also becoming 3D with sophisticated gestural and tracking technologies. 
% In the same way, the ``recorded video'' is also shifting from 2D to 3D --- with the more-accessible depth camera or LiDAR sensor, now we can capture and record our environment as 3D as opposed to 2D video in much easier ways.
% Such videos are often called ``volumetric video'' [cite], which captures the video as a point-cloud 3D data of the scene so that the user can see the content as in 3D. 
% In fact, such volumetric videos are increasingly becoming in many different application areas, such as live performance [cite], sports training and analysis [cite], entertainment [cite], tutorials [cite], and beyond. 
% Given this trend along with the technological advances of camera devices, it is almost inevitable that the next generation of consumer video platform will become 3D, where people watch 3D volumetric videos on YouTube, Instagram, or TikTok in the everyday scenarios.




% the viewing experience of volumetric videos has not been changed at all --- we just watch 

% However, today's volumetric videos research and commercial products only focuses on \textit{capturing and viewing} aspects, but \textit{editing} aspect still remains far behind --- it becomes much easier to record or play these volumetric videos with devices like Kinect, we still do not have an appropriate ``editing tool'', as opposed to a lot of sophisticated tools for 2D videos like Adobe Premiere or Final Cut Pro. 

% Using augmented video to test in-car user experiences of context analog 

% in the captured and reconstructed 3D scene, volumetric videos, either live or recorded, are changing the viewing experiences in many applications such as live performance [cite], sports training and analysis [cite], entertainment [cite], tutorials [cite], and beyond.
% provide editing tools for volumetric video. However, these tools only allow simple timeline manipulation and does not provide any visual effects editing or annotation. 
% With the recent proliferation of depth cameras (e.g., Kinect), 3D volumetric capture became easier and more ubiquitous than ever before. 
% However, it's not well-supported with 3D volumetric videos 
% However, unlike 2D videos which have a lot of editing and annotation tools and augmented video examples, the current volumetric videos mostly focus on just watching the reconstructed 3D scene as is the real-world.



% allows the simple authoring of embedded and responsive visual effects that 
% We call this and 
% Our system leverages the object-bound annotation approach, which can significantly reduces the time and cost for volumetric video editing. 

% as if 



% based on the object motion and body movements. 
% o that the sketched elements dynamically move with the corre- sponding physical motion. 

% visual effects 
% sketches on a phone or tablet screen, which embeds interactive visualizations into a scene. The sketched elements can be bound to physical objects such that they respond dynamically as the real world changes.
% edit and augment 3D volumetric videos with object-centric annotation and visual effects. 

% Our system leverages the object-bound annotation approach, which can significantly reduces the time and cost for volumetric video editing. 
% For example, Figure 1 illustrates that what the user can create with Recorded Reality system.
% The user can easily select an object on the scene then the system automatically tracks the object in 3D space, so that the user can embed visual effects, annotation, and visualization in the scene without programming. 



% by introducing a new way to augment captured physical motion with embedded and responsive visual effects, which we call \textit{object-centric augmentation}. 
% which we have compiled as an interactive gallery1. Our analysis based on the collected videos suggests the importance of speech modality for a variety of interactions. Based on the observed common augmentation tech- niques, we identify the design space for augmented presentations: 1) textual elements (e.g., title, keywords, and list), 2) associated visual elements (e.g., images, icons, and screens), 3) location of the elements (e.g., in front of the presenter, 3D surface, and physical object), 4) interactions with the elements (e.g., drag and drop, and scaling).
% contribute to a taxonomy of such .

% , which include . 
% , whose designs are informed by the analysis of 120 video-edited object-centric visual effects. 

% conducted two user-centered approach: 1) a formative interview with four professional volumetric video editors, 2) analysis of existing video editing practices.
% Through the study, we identify that the editing of the current 3D volumetric video is very time-consuming tasks, and identify three design goals of the system, based on the most common use cases and needs for the volumetric videos: 1) xxx, 2) xxx, 3) xxx. 
% In addition, we have also analyzed the common techniques and practice of video editing and augmentation. Given that, we have identified the system design for the Recorded Reality.


 
RELATED WORK


% Reality Sketch
% Soccer on a Tabletop:
% Sport Analysis: EventAnchor
% There are many promissing applications with using our tool
% \begin{figure*}[h!]
% \centering
% \includegraphics[width=250px]{figures/related_work.png}
% \caption{Related Work}
% \label{fig:related-work}
% \end{figure*}
% Commercial Products: Adobe Premiere, 2D vs 3D.
% The commercial products for 3D, simple manipulations, in contrast
% In the research field, reality sketch, body-driven augmentation (2D video vs Volumetric). Why we need to have different techniques for vol, vol need different techniques because ... (3D video annotation is volumetric, manipulating space and time, not alinged to the object). ---- we cannot directly use the existing tools, that's why we need Recorded Reality.

% Understanding Newcomers to 3D Printing --- Why 3D is harder than 2D and why we need Recorded Reality

%  Lastly, there are also some research work focusing on volumetric capturing and 3d video processing of volumetric video \cite{schreer2019capture}, however, these works still stay on a primitive level of meshing [cite], digital human modeling [cite] and body animation [cite].

% In contrast to prior work on augmented reality and available products, we do not show users a simple camera image of the physical world but a 3D reconstruction of their environment. This enables changing the physical world as easily as the virtual world, which is challenging with typical augmented reality techniques.

% SceneCtrl:
% LiDARMan:












% \subsection{Volumetric Video Editing Tools}

% Volumetric video is regarded worldwide as the next important development step in the field of media production. Especially in the context of the extremely rapid development of the Virtual Reality and Augmented Reality markets, volumetric video is becoming a key technology.


% To the best of our knowledge, no existing works have explored this approach.
% This design decision is backed up by the analysis of existing video-edited augmentations where we found that many of the video augmentation is triggered based on the presenter's speech. 


% meshing and mesh
% reduction algorithm finally produces a sequence of meshes
% that can be integrated into common render engines.


% \subsection{3D Scene Reconstruction}

% \subsection{Embedded Annotations and Visualizations}

% \jian{This whole subsection is under construction}
% \jian{Reality Sketch, Soccer on a Tabletop, Sport Analysis...}





% An alternative approach is diminished reality or illusionary transparency [23, 24, 25] which usually focuses on removing objects from a video feed. Typically, erasing requires infer- ring the environment behind the object through inpainting [11], approximation [52], or using multiple cameras as in our implementation. 


% \jian{This subsection is still under construction}

% Aforementioned work focused on interaction on static data. Therefore, manipulation performed in one frame would be lost in the next frame. In our implementation, users perform selections and manipulations on an underlying voxel grid, which enables consistency across frames.

% Volumetric videos is considered a step forward towards an immersive photo-real experience. That is, it incorporates mixed reality but has the realism by reflecting the real world. Unlike virtual reality that uses computer graphics or rendered models. As it is a newer field and can be considered relatively unexplored, there is much room for improvement. Earlier works and studies have been done to describe the process of volumetric capture and techniques on optimization[Paper 3 and 4 from Gdoc] (Expand/discuss work more?). These papers incorporated the usage of voxels. But in our case, we will focus on point clouds. (elaborate and then flow into methods of tracking?)







% Commercial tools, like Canvas [37] or Polycam [25] on the iPhone 12 Pro and the Microsoft Hololens, as well as research like 
% KinectFusion [26] and DepthLab [10], have significantly low- ered the barrier of entry to accessing environmental geometry data.

% to enable 
% A volumetric video appears like a video and can be played back and viewed from a continuous range of viewpoints chosen at any time. 
% A number of techniques have been proposed to synthesize point- and surface-based free-viewpoint video (FVV), including shape from silhouettes [Ahmed et al. 2008; Wu et al. 2011], freeform 3D reconstruction [Liu et al. 2009; Vlasic et al. 2009] and deformable models [Carranza et al. 2003].
% More accessible volumetric capturing 
% 3D reconstruction of a sense has been used for a long time to generate virtual representations of real scenes. An early example is Virtualized Reality by Kanade et al. [30]. With the increasing availability and quality of RGB-D cameras, many researchers have investigated high-quality reconstruction approaches [8, 9, 28, 72]. 
% \subsubsection{Remote Instruction}
% capturing 3D data of a remote environment also has applications in remote instruction 


% uses AR and virtual avatar to immersive tutorial instructions for machine and mechanical task.

% LIDARMAN~\cite{miyaki2016lidarman}
% and remote collaboration





% For example,  use real-time 3D reconstruction for remote collaboration on physical tasks
% Teo et al.~\cite{} combine 360 video and 3D reconstruction for mixed reality collaboration
% Alternatively, 
% Previous works also  techniques to render parts [50] or all of the physical environment, e.g., for telepresence [19]
% the recent advances in RGB-D cameras,
% \subsubsection{Telepresence and Remote Collaboration}
% For example, the past work demonstrates the virtual telepresence through 3D teleportation (e.g., 
% For remote collaboration 




% With Fusion4D, Dou et al. [cite] performed reconstruction on live data, however their approach does not work for large motion such as a user moving through a room. 
% These approaches focus on mapping and reconstruction of environment rather than user interaction. Scheiblauer and Wimmer [cite] used volumetric representations to perform selection in large scale point clouds. Owada et al. [cite] introduced the “volume catcher,” which allows users to select regions on a 3D mesh through 2D contours. 

% Lidarman [cite] enables live out-of-bo・y experiences by presenting users with a reconstructed view of a head-mounted light and range detection sensor. Remixed Reality uses external cameras to increase the range of possible viewpoints and enlarge the space of possible manipulations. Photoportals [cite] allow users to record remote and local content, and review it in an immersive environment. 
% On a technical level, our approach relies on the ability to interact with the virtual environment and to manipulate it. 
% KinectFusion [cite], as one example, tracks the environment and refines a model by matching consecutive frames of depth data. 



% \subsubsection{Object Detection in Volumetric Capture}
% object detection and semantic segmentation,  has enabled applications to obtain a semantic understanding of the user’s physical surroundings.
%  usees this information tocreate context-aware application 

% SemanticPaint~\cite{valentin2015semanticpaint}
% \subsubsection{Timeline Interaction Techniques}
% \subsubsection{Spatial Interaction}




% Valentin et al. [cite] extended this approach with segmentation. 
% Innmann et al. [cite] fit a model to the received depth data to accurately reconstruct volumetric deformation. 
% Singh et al. [cite] used skeleton data from meshes to infer possible selections. 
% Bürger et al. [cite] introduced manipulation techniques for volumetric data based on scalar fields. While we also use a volumetric representation, we focus on live data, i.e., the mesh changes every frame.


% or replacing the physical object , 
% erase 
% SceneCtrl~\cite{yue2017scenectrl} erase objects from the physical scene 
% With SceneCtrl, Yue et al. [cite] perform spatial changes in the environment (erase, copy, move) based on 3D reconstruction and display them with an optical see- through display (Microsoft HoloLens). 
% Their approach relies on a static mesh generated during reconstruction, whereas changes performed with Remixed Reality apply to live geometry (e.g., a copied object and its source will both move if the source moves).

% The immersed user sees a version of the whole room with several space-time modifcations applied (e.g., moved or copied ob- jects). The system features immersive recording and playback of point clouds, yet is oblivious to individual people, objects, their
% Remixed Reality \cite{lindlbauer2018remixed} does the 3d reconstruction using multiple Kinect camera providing a room-scale live experience, however remixed reality focuses on live reconstruction and 


% that can be used for a wide range of applications,


% the idea of visually enhanced volumetric capture (e.g., Remixed Reality)
% Along with the novel direct manipulation authoring, \system{} extends the idea of previously explored volumetric augmentation (e.g., Remixed Reality~\cite{lindlbauer2018remixed}) to support more comprehensive visual effects that can be used for a wide range of applications,
% However, these works only allows the simple transformations such as copy and deleting an object. 
% In contrast, Recorded Reality focuses on the post-processing of the volumetric capture by leveraging object-bound approach to edit and add visual annotation effects which is bound to the object.


% Most approaches that focus on depth data either rely on static geometry or continuously refine geometry that is assumed to be static. 

% Traditional video editing tools such as Adobe Premiere Pro or Final Cut Pro are tailored towards 2D videos editing instead of 3D, which leaves a considerable gap remained in the market for volumetric video editing. In recent years, there appears some commercial tools for volumetric video editing, such as 4Dfx \cite{4dfx}, DepthKit Studio \cite{depthkit} or HoloEdit \cite{holoedit}. 
% However, these tools only provides simple timeline manipulations and focuses on the meshing and texture effects of the captured objects. 
% Prior works relating to temporal manipulations such as video playback in mixed reality has already been explored. 
% These works either use 3D interfaces or object manipulation for time navigation. 
% However there has yet to be an incorporated system that has manipulations to cut out scenes or rather essentially skipping over periods of time. Much like cutting or splicing clips from videos.
% Mixed Voxel Reality~\cite{regenbrecht2017mixed} 



% such as object, text and geometric shapes to 3D anchored position of tracked object within volumetric videos and further create annotative edits such as highlighting and simple visualizations.


% This limitation of the public accessibility and creative freedom has potentially blocked the media creation and consumption for the general public regarding the volumetric videos.


% , classroom education (RealitySketch~\cite{suzuki2020realitysketch}), storytelling (Interactive Body-Driven Graphics~\cite{saquib2019interactive}), interactive data visualization (), live presentation (), and entertainment ()
% \subsubsection{Authoring Interfaces}
% RealitySketch~\cite{suzuki2020realitysketch}

% Video Summagator~\cite{nguyen2012video}: An interface for video summarization and navigation


% Direct Space-Time Trajectory Control for Visual Media Editing


% in the context of remote collaboration,  allows the sketched annotation for AR scene
% Direct Manipulation Video Navigation in 3D
% Direct Manipulation Video Navigation on Touch Screens~\cite{nguyen2014direct}
% Adaptive Video Playback Based on User Motion for Supporting Physical Activity
%  A Direct Manipulation Video Navigation Interface for Mobile Devices
%  Direct Manipulation Keyframe Timing for Performance-based Animation


% Cliplets~\cite{joshi2012cliplets}: Juxtaposing Still and Dynamic Imagery
% In particular, many works leverage object-centric approaches  
% (e.g., PocketDRAGON~\cite{karrer2009pocketdragon}, DRAGIMATION~\cite{walther2012dragimation}, Nguyen et al.~\cite{nguyen2013direct, nguyen2012video, nguyen2014direct}, Santosa et al.~\cite{santosa2013direct}), 
% Real-Time Annotation of Video Objects on Tablet Computers

% Goldman et al.~\cite{goldman2008video}
% Video Object Annotation, Navigation, and Composition

% However, these techniques are only discussed in 2D videos, it is necessary to introduce different editing techniques for volumetric videos, because annotation and editing in 3D volumetric videos are inevitably more challenging when manipulating space and time [cite] or aligning the 3D objects \cite{hudson2016understanding}.

% In this section we will discuss the prior works related to volumetric capturing and annotative editing for volumetric videos. We will also clarify techniques used for 3D scene reconstruction and object tracking used for embedded annotations.


% reducing human interactions in event annotation of racket sports videos
%  explores a VR environment that can easily bridge in-situ and ex-situ visual analytics

% Slicing-Volume~\cite{montano2020slicing} explores a selection technique for volumetric point-cloud data. 
% posture 
% human movement annotation posture
%  immersive analysis for human motion data and trajectories
% immersive visualization of game player's motion data~
% and 


% HeatSpace and OptiSpace not only visualize but also optimize the user interface÷
% Researchers have also explored ways to help people annotate video data through interaction designs. One research direction is to explore new interactive approaches to facilitate important annotation
% tasks, such as an adaptive video playback tool to assist quick review of long video clips [cite], a mobile application to support real-time, precise emotion annotation [cite], an interaction pipeline
% for the annotation of objects and their relations [cite], and a novel
% method to acquire tracking data for sports videos [cite]. These designs, which largely target single users, can improve the efficiency and accuracy of video annotation from different perspectives. 
% Various tools [cite] have been developed for video data
% annotation. Early work largely focused on object recognition and
% annotation. For example, ViPER [cite] can annotate the bounding
% boxes of objects and texts frame by frame, and LabelMe [cite] supports the annotation of the same object across different frames. As
% the demands for video annotation dramatically increased, efforts
% were made to reduce the burdens in the annotation. VATIC [cite],
% for example, was designed to leverage crowdsourcing for video
% annotation; iVAT [cite] combined automatic label generation with
% user manipulation to improve annotation efficiency; ViTBAT [cite]
% supported the annotation of individual and group behaviors across
% different frames.

%  allows the activity annotation with skeletonized surveillance videos
% Review paper~\cite{choudhary2016video}
% Alternatively, provides a mixed reality toolkit for spatio-temporal data visualization

% visualizing surveilance videos
%  analyzes for visualizing spatial interactions in the physical environment.
% Sugito et al. explores browsing group first-person videos with 3d visualization
% Yu et al.~\cite{} explores motion guidance in mixed reality


% Kloiber et al.~\cite{kloiber2020immersive} also work on immersive analysis of user motion in VR environments


FORMATIVE STUDY
% \section{Volumetric Video Editor Interview}
% Our overall goal was to elicit the design goals for editing 3D volumetric videos in order to derive design guidelines for a volumetric video annotative editing system. 

% \subsection{Target Annotative Editing Effects}
% Here we identify the target effects that we asked the volumetric video editors to reproduce.

% \subsubsection{Adding Object}
% Adding an object (visuals, 3D models etc) to the volumetric video, which could be anchored in a 3D position or attach to another 3D object which is following with the movements.

% \subsubsection{Adding Text}
% Adding a text to the volumetric video, which could be placed on 3D surfaces or in the mid-air, the text could be dynamic to the motion tracking values.

% \subsubsection{Adding Geometric Shapes}
% Adding geometric shapes, such as line, angle or area to the volumetric video.

% \subsection{Participants}
% We recruited four professional volumetric video editors, (3M, 1F) aged 25 to 58 (median 42). All participants had a minimum of two years of experience creating volumetric videos. Participants had diverse backgrounds in 2D video editing, 3D character animation, motion graphics, and digital human modeling. Participants had experience with numerous software packages including After Effects, Maya, Blender, Character Animator, Apple Motion, Toon Boom Harmony and Unity.
% For the four volumetric video editors (P1–P4), we conducted an initial session with the first three target effects. The study took between 75 and 120 minutes.

% \subsection{Apparatus and Procedure}
% Participants were appointed the same volumetric videos for the editing by providing the Kinect captured ``.ply'' files. We then asked the participants to recreate the target annotative editing effects using their familiar tools, such as Unity or Blender. In each session, we presented target effects to the participant. For each example, we started by showing the static scene objects and then playing the target eding effects.

% \subsection{Results}
% We identify three design goals of the system, based on the most common use cases and needs for the volumetric videos: 1) xxx, 2) xxx, 3) xxx. 





% \subsection{Initial Findings and Design Rationale}
% Our initial findings with the collected edited videos suggest the objects (object and body) in the video plays a critical role in triggering a range of visual and textual elements as annotations. 
% Therefore, in our system, we decided to explore this \textbf{\textit{object-bound approach}} as the primary modality for the users to edit their volumetric videos, and create our editing tool and editing techniques centered around the object during the post-processing time. 
% In the following section, we further categorize the design space of this object-bound annotative editing effects.
% In these videos, we identified at least one scene with embedded or augmented elements based on or related to the presenter's spoken keywords. 
%This is a natural interaction flow as the augmented presentation often leverages the spoken narrative by the presenter and it is a natural decision to add the visual or textual aid based on the keyword that the presenter just says. 



% In Recorded Reality, the user can bind the 3D visual elements such as objects, text, and geometric shapes to the body or tracked objects. 
% With that, the user can easily create a visual effects like highlight or annotation with much easier way without thinking about 3D manipulation.
% The user can also translate or transform these elements based on the body or object movement in 3D space, so that the user can visualize these motion. 
% Finally, the user can also track the motion data based on the object tracking for 3D embedded visualization like heat map or graphs.
% By combining these available features, the user can create a lot of different augmented scenes for 3D volumetric videos. 

% Recorded Reality employs the 3D volumetric capturing with multiple Azure Kinect cameras and provides an interface based on A-Frame and Three.js. By capturing and recording the volumetric scene, the system reconstructs the scene with colored 3D point-cloud.
% In addition, we track the object by leveraging both computer vision and depth information.


% contain edited annotative effects from different application areas where the objects are usually bound with visuals, texts, annotations and visualizations. 

% \jian{Fig. Collected Examples}

DESIGN SPACE

% of the videos is not the systematically collected examples nor the 
% for the augmented presentation. 
% After this process, two authors performed systematic coding with individual tagging for categorization of the complete dataset. 
% Finally, we reflected upon the individual tagging to resolve the discrepancies to obtain the final coding results.
% \subsubsection{Methodology}
% % The criteria for our augmented presentation search include
% After the filtering process, we have identified 150 videos and images for our analysis. 

% We first tried to collect with a systematic search result based on a specific keyword like , but we did not obtain meaningful results mostly

% because 1) there is no common keyword associated with these 3D edited volumetric videos to date, 2) example videos or annotative effects are often used for different context or purposes.
% Therefore, we collected these videos mostly based on manual visual search using visual search platforms like Pinterest or Google Image Search. 





SYSTEM


% \subsubsection{Translation}
% \subsubsection{Color Changes}
% \subsubsection{Opacity Changes}
% \subsubsection{Scale}
% \subsubsection{Rotation}
% \subsubsection{Speed}


% \subsection{Features}
% Given the analysis of the design space (Elements, Placement, Movement, and Transformation), we present the system features for annotative editing in volumetric videos.
% % elements, design space


% \subsubsection{Element Binding}
% Placement -> Bound + Movement -> Following + Geometric Shapes (Line)

% \subsubsection{Animation}
% Movements -> Active + Time / Locomotion

% \subsubsection{Trajectory}
% Locomotion + Time

% \subsubsection{Highlighting}
% Color Changes + Opacity Changes

% \subsubsection{Ghost Effect}
% Cloned Object + Color Changes + Opacity Changes + Locomotion

% \subsubsection{User-Defined Data Collection and Visualization}


% \section{Design Space of Object-Bound Approach}
% In this subsection, we present the design space of the object-bound approach through our formative interview and the analysis of the collected edited videos. In Figure 3, we have analyzed and identified the design space as the following four levels: 1) Elements,
% 2) Placement, 3) Movement, and 4) Transformation. 

% \jian{Fig. Design Space}


% \subsection{System Walk-through}
% step 1, step 2, step 3 ... (Sketched Reality)
% show how the system walk-through the user to create
% select one example with multiple features

% describe how the user can recreate the effects (tutorial)




% \section{Recorded Reality}


% \section{Recorded Reality}


% \subsection{System Overview}
% \jian{Fig. System Workflow}

% \subsection{Demonstrating Recorded Reality}

% \begin{figure*}[h!]
% \centering
% \resizebox{\linewidth}{!}{
% \includegraphics[height=1\textwidth]{draft-figures/0.JPG}
% \hspace{0.5cm}
% \includegraphics[height=1\textwidth]{draft-figures/1.JPG}
% \hspace{0.5cm}
% \includegraphics[height=1\textwidth]{draft-figures/2.JPG}
% }
% \caption{System Usage}
% \label{fig:system-usage}
% \end{figure*}

% \subsubsection{Interaction Workflow and Techniques}

% \subsubsection{Select Objects and Create Binding}

% \subsection{Place the Objects}



% % \subsubsection{Bound}

% % \subsection{Movement}
% % Movement refer to the position changes of existing objects. Based on the analysis, we identify the movements could be: 1) Active, 2) Passive, and 3) Following.
% % \subsubsection{Active}
% % Active means the object movements are self-actuated based on time or a given path, for example, a virtual cloud that is embedded into the scene that floats around.
% % \subsubsection{Passive}
% % Passive means the movements are driven by other motions, for example, the user pushes away the cloud or grab the cloud towards them.
% % \subsubsection{Following}
% % Following is essentially the object movements are bound to another object.
% % \subsection{Viewpoint}
% % Changing the viewpoint similar to JackInSpace.
% % 
% \subsection{Transformation}
% Transformation refers to a series of changes to the parameters of the objects, including: 1) Translation, 2) Color Changes, 3) Opacity Changes, 4) Scale, 5) Rotation, and 6) Speed.





% \subsection{Binding Locations}
% \subsubsection{Environment}
% \subsection{Dynamic Parameters}
% \subsection{Design Components}
% .
% \subsubsection{Object}
% \textit{New Object} refers to the object asset (visuals, 3D models, etc) that can be added into the scene manually, for example, adding a virtual ball to the table tennis scene. Or it could be the object that is brought into the scene while recording; \textit{Cloned Object} specifically refers to a cloned object which is like ``copy and paste'' from the existing object in the scene.
% \jian{Fig. Object}
% \subsubsection{Text Mesh}
% \jian{Fig. Text}
% \jian{Fig. Geometric Shapes}
% \subsubsection{Locomotion}
% \subsubsection{Parameters}
% \subsection{Placement}
% \subsubsection{Static}
% Static refers to a static placement to an 3D anchored position which doesn't change throughout the volumetric video.


SYSTEM


% Recorded Reality is a tool for editing volumetric videos, informed by the analysis of the existing video-edited examples. 



% an augmented reality interface to embed responsive graphics and visualizations through real-time dynamic sketching.
% draw dynamic sketches based on the user-defined specification:
% the user can simply select and bind captured physical objects with annotated visual effects. 


% mobile augmented reality (ARKit) to embed sketches in the real world. The user sketches with a finger or a pen on a touchscreen, where the sketched elements are overlaid onto a camera view of the real world (Figure 5).

% Rather than 2D sketches that are based on the device screen coordinates, all sketched elements have a 3D geometry and position in real world coordinates, anchored in 3D space. This way, the user can move the device to see from a different perspective and the sketches stay correctly anchored to the real objects. To enable this functionality, our system leverages ARKit and SceneKit for both surface detection and object placement in the 3D scene. Therefore, the first step is to detect a horizontal or vertical surface, as all interactions (e.g., tracking an object, sketching elements, placing a graph) are based on a reference surface in a 3D scene. Once the surface is detected, the user can start using the system. In RealitySketch, the user can sketch on both real-time and prerecorded scenes. For real-time sketching, the user can just start sketching once the surface detection is finished. For recorded scenes, RealitySketch first allows users to capture and record the video with an internal recording feature. The recorded video is embedded with additional meta information at each time frame, such as the current camera position, the current origin point, and the position of detected surface. Based on this recorded information, RealitySketch can reconstruct the 3D scene, which is associated with the recorded camera view of each time frame. Thus, the user can sketch, annotate, or visualize on top of the RealitySketch’s recorded video, while controlling the timeline of the internal video player. Due to these constraints, this recording feature does not work with conventional videos.



% . Therefore, the tracking feature best works with dis- tinct, solid colors. Based on this detected mask, the system obtains the largest contour and computes a center position of the tracked object on the screen. The system then converts these 2D coordinates into the 3D world coordinates by ray casting the 2D position onto the detected surface, assuming that the tracked object moves onto the detected horizontal or vertical surface. This color tracking was fast enough for most of our applications (e.g., 20-30 FPS with iPad Pro 11 inch 2018). The user can also use the joint of the human body as additional tracked objects. In this case, we use ARKit 3’s built-in human motion tracking feature that gives us the 3D position information of the body joints.



% Placement refers to where the elements could be placed into the volumetric video. Based on the analysis, we identify the placements could be: 1) Static, 2) Bound.

% For embedded and responsive graphics, the graphical elements need to be tightly coupled with physical objects and environments. Thus, capturing and tracking an object is vital to make the graphics dynamically change and move. To specify an object, the user enters the selection mode and then taps an object on the screen (Figure 6A). Once selected, our system highlights the selected object with a white contour line (Figure 6B) and starts tracking the object in the 3D scene (Figure 6C).



% \subsubsection{Object}
% An object refers to the existing objects that are captured in the scene, we identify the objects can be a scene object or human body.
% In addition the existing objects, we also identify external objects that can be embedded into the volumetric video, which could be anchored in a 3D position or attach to another object which is following with the object movements. The external objects can be either ``New Object'' or ``Cloned Object''.
% \subsubsection{Body}

% \subsubsection{Surface and Environment}


% The system then automatically tracks physical objects such that the embedded visual effects can move and respond dynamically with the corresponding physical motion and body movement.
% This approach, which we call \textit{object-centric augmentation}, can significantly reduces the time and cost of the creation of augmented volumetric videos.
% In addition, unlike 2D videos, the augmented 3D scene allows free-viewpoint movement, which enable the immersive viewing experiences.

% \item Bind the real-world parameters into existing graphics to make the graphics responsive.




% A text is also considered to be an object, which can be embedded into the volumetric video. We identify text as a high-level element because text is the most common annotative techniques such as labeling an object. 


% And similarly, it could also be placed on 3D surfaces or in the mid-air. The text could either be Static Text or Dynamic Text to dynamic values.
% \textit{Static Text} refers to the value of a text element that doesn't change or modify consistently throughout the volumetric video.
% \textit{Dynamic Text} refers to the value of a text element that is changing responsively to a dynamic value, such as motion and time.



% Bound refers to a binding placement with an existing object's position which follows the movements of the object, which could either be bound to an object or human body.


% \section{Implementation}

% \subsection{Volumetric Capturing}

% \subsection{Object Tracking in 3D}

% \subsection{3D Reconstruction}

% \subsection{User Interface}



% ased on the user-defined key- words, the presenter can further augment the presentation based on the prepared or improvisational associated visual information. As we discussed in the authoring tool section, For example, Figure 6 illustrates the presenter can show three photos based on the keywords or show a QR code based on a user-defined trigger word. These visual elements are also interac- tively manipulated with gestural interaction (described below) so that the user can make it more interactive.

% gure 7 also illustrates how the user can also add the screens based on the specified URL. For example, the user can show a Google or Wikipedia screen as the embedded iframe element. 

% \(f(t) = (x,y,z)\). \(f(t)\) is a function that tracks the \((x,y,z)\) position of any selected object within the volumetric video based on time. This is the fundamental component to support the annotative editing effects that can be anchored to a 3D position \((x,y,z)\) or bound to an object that follows the movements. Furthermore, given any timing of  \(t0\) and \(t1\), we can derive the speed of the object by just simply do \(distance / (t1 - t0)\).


% \subsubsection{Geometric Shapes}



% \subsubsection{Volume} 
% Geometric shapes refers to simple geometry that can be embedded into the volumetric video, such as line, angle or area.
% Parameters refer to the attributes of the objects within volumetric video, namely position, color, opacity and size.

% define and capture the dynamic value of interest. In this paper, we specifically focus on parameterization that can be done through simple sketching interactions using line segments. Line segments are one of the most basic sketching elements, which are commonly leveraged in the existing interactive sketching systems (e.g., [33]). Line segments are useful as they work alone to parameterize a length between two points, but also can be combined to define different parameters, such as an angle between lines or an area of a closed geometric shape. They can also be used for annotated lines or guided lines. The user could also draw a simple 3D diagram with these line segments like [32], which could be used as a responsive visual output itself. Here, we describe how this line sketching interaction can define and capture the dynamic value of interest. First, when entering the sketching mode, the user can start drawing a line segment onto the scene (Figure 7A). All the sketched lines are projected onto a 2D surface within the 3D scene. The system takes the two end-points to create the line segment. This creates a variable that defines the distance between two points on the surface. To create a dynamic line segment, the user draws a line whose end point is attached to the selected object (Figure 7B-C). As one end of this dynamic line segment is bound to the selected object, if the user moves the object in the real world, the line segment and its parameter (e.g., distance value) will change accordingly. The system visually renders the line segment values using labels.



% Similarly, the user can define a constraint by typing a function of existing variable. For example, consider the user wants to draw the bisector of the angle formed by a dynamic line segment. The user can first draw a line and an arc between the line and the base line (Figure 11A). Then, the user taps the label and types angle/2 (Figure 11B). Then, the system can recognize the function to dynamically bind the parameter to be half of the existing parameter (Figure 11C). In a similar manner, the user can also change the length or distance of the sketched elements with a function (e.g., the force of a spring in Figure 4). In our current implementation, the system can parse basic arithmetic operations, trigonometric functions, and polynomial expressions.

% RealitySketch can also make responsive visualization based on graph plotting of a parameter. In the graph placing mode, the user can place a 2D graph and change its size by dragging and dropping onto the surface. By default, the x-axis of the graph is time. By binding an existing variable to the graph, it starts visualizing the time series data of the variable.  To bind the variable, the user can simply tap a label of the graph (Figure 12A), and then, enter the variable the user defined. For example, if the user binds the angle variable of the pendulum to the y-axis of the chart, the graph will dynamically plot the angle of the pendulum when it starts swinging (Figure 12B-C). By adding multiple variables separated with a comma (e.g., a,b, c), the user can also plot multiple parameters in the same graph. The user can also change the x-axis from time to a variable by tapping the x-axis and entering a second variable. For example, the user can define an angle and y distance of a point of a circle. By binding x-axis as the angle and y-axis as the perpendicular length, the system can plot the relationship between the angle and corresponding sine value (e.g., Figure 14).


% To make the existing line segments responsive, the user can bind variables between two elements. The parameter of a static line segment can be bound to another variable. For example, suppose the user has a variable named angle for a dynamic line segment. When the user taps the label of another angle of the static line segment (Figure 10A), the system shows a popup to let the user enter the variable name. If the entered variable name matches an existing name (e.g., angle in this case), the angle of the static line segment will be dynamically bound to the existing parameter (Figure 10B), so that when the angle value changes, the angle of another line is also changed (Figure 10C). This works as a dynamic constraint between multiple line segments.



